Moment polytopes for symplectic manifolds with monodromy

A natural way of generalising Hamiltonian toric manifolds is to permit the presence of generic isolated singularities for the moment map. For a class of such ``almost-toric 4-manifolds'' which admits a Hamiltonian $S^1$-action we show that one can associate a group of convex polygons that generalise the celebrated moment polytopes of Atiyah, Guillemin-Sternberg. As an application, we derive a Duistermaat-Heckman formula demonstrating a strong effect of the possible monodromy of the underlying integrable system.

==> macro.tex <==
% macros Vu Ngoc San

%requires package amsmath
\RequirePackage{amsmath}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pscal}[2]{\langle #1,#2\rangle}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\formel}[1]{[\![#1]\!]}
\newcommand{\ham}[1]{\mathcal{X}_{#1}}
\newcommand{\Lie}[1]{\mathfrak{#1}}
\newcommand{\ad}[1]{{\operatorname{ad}}_{#1}}
\newcommand{\Ad}[1]{{\operatorname{Ad}}_{#1}}
\newcommand{\Aut}{\mathop{\operatorname{Aut}}\nolimits}
\newcommand{\re}{\mathop{\mathfrak{R}}\nolimits}
\newcommand{\im}{\mathop{\mathfrak{I}}\nolimits}
\newcommand{\mbold}[1]{\textnormal{\boldmath{$#1$}}}

\newcommand{\phy}{\varphi}

\newcommand{\ssi}{\Longleftrightarrow}
\newcommand{\impliq}{\Rightarrow}
\newcommand{\fleche}{\rightarrow}
\newcommand{\inject}{\hookrightarrow}
\newcommand{\restr}{\upharpoonright}
\newcommand{\bigrestrs}[1]{\left.#1\right|\hspace{-7.22pt}\upharpoonright}
\newcommand{\bigrestrr}[1]{\left.#1\makebox[0ex]{\hspace{3.7pt}$\upharpoonright$}\right|}
\newcommand{\trsp}{\raisebox{.6ex}{${\scriptstyle t}$}}
\newcommand{\limi}[1]{\displaystyle \lim_{#1}}
\newcommand{\tr}{\mathop{\operatorname{tr}}\nolimits}
\newcommand{\rem}[1][$\!\!$]{\noindent {\sl ${\mathcal{R}}$emark #1. }}
\newcommand{\egdef}{\stackrel{\mathrm{def}}{=}}

\newlength{\Taille}

\newcommand{\flechedroite}[1]{%
  \settowidth{\unitlength}{\mbox{$#1$}}
  \settoheight{\Taille}{\mbox{${\scriptstyle #1}$}}
  \addtolength{\Taille}{1ex}
  \addtolength{\unitlength}{4ex}
  \raisebox{0.5ex}{%
  \begin{picture}(1,0)
    \put(0,0){\vector(1,0){1}}
    \put(0.5,0){\makebox(0,0){${\scriptstyle #1}$ \vspace{\the\Taille}}}
  \end{picture}}}


\newcommand{\cqfd}{\hfill $\square$\par\vspace{1ex}}
\newcommand{\finex}{$\diamond$}
\newcommand{\finrem}{\hfill $\oslash$}
\newcommand{\dens}{\Omega_{\frac{1}{2}}}
\newcommand{\Cinf}{C^\infty}
\newcommand{\COT}[1]{T^* #1 \setminus\{0\}}
\newcommand{\intint}{\int\!\!\!\int}
\newcommand{\gener}[1]{\langle #1 \rangle}
\newcommand{\ind}{\mathop{\operatorname{Ind}}\nolimits}
\newcommand{\coker}{\mathop{\operatorname{Coker}}\nolimits}

\newcommand{\RM}{\mathbb{R}}
\newcommand{\ZM}{\mathbb{Z}}
\newcommand{\QM}{\mathbb{Q}}
\newcommand{\NM}{\mathbb{N}}
\newcommand{\CM}{\mathbb{C}}

\newcommand{\T}{\mathbb{T}}

\newcommand{\PM}{\mathbb{P}}
\newcommand{\LM}{\barre{L}}

\newcommand{\B}{\mathcal{B}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\A}{\mathcal{A}}

\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}

\newcommand{\theor}{Theorem}
\newcommand{\defin}{Definition}
\newcommand{\lemma}{Lemma}
\newcommand{\remar}{Remark}
\newcommand{\corol}{Corollary}
\newcommand{\propo}{Proposition}
\newcommand{\demon}{Proof}
\newtheorem{theo}{\theor}[section]
\newtheorem{theo*}{\theor}

\newtheorem{defi}[theo]{\defin}
\newtheorem{prop}[theo]{\propo}
\newtheorem{lemm}[theo]{\lemma}
\newtheorem{coro}[theo]{\corol}
\newtheorem{conj}[theo]{Conjecture}
\newtheorem{prob}[theo]{Problem}

\newcommand{\demons}[1][$\!\!$]{\noindent\textbf{\demon\ }\textsl{#1}\textbf{.}~}
\newenvironment{rema}
{\par\vspace{1ex}\refstepcounter{theo}%
\noindent\textbf{\remar~\thetheo} }
{\penalty 500\hfill\mbox{$\triangle$}\par\vspace{1ex}}

% environement ``hypothese'':
\newcounter{hypo}
\setcounter{hypo}{0}
\def\thehypo{\textbf{\textup{(H\arabic{hypo})}}}

\newenvironment{hypo}
{\refstepcounter{hypo}%
\begin{center}\thehypo.\hfill\begin{minipage}{.9\linewidth}}
{\end{minipage}\end{center}}

% demo
\newenvironment{demo}[1][$\!\!$]
{\demons[#1]\ }
{\cqfd}

%environement liste continue (enumerate avec continuite des numeros)
\newcounter{listcont}
\setcounter{listcont}{0}
\def\thelistcont{\arabic{listcont}}

\newenvironment{listcont}
{%\refstepcounter{listcont}%
\begin{enumerate}\setcounter{enumi}{\thelistcont}}
{\end{enumerate}\setcounter{listcont}{\arabic{enumi}}}


% pour la typographie des adresses URL
\newcommand{\ellastiq}{\hspace{0pt plus 0.5ex}}

%la convention standard pour les footnotes est debile en math:
\renewcommand{\thefootnote}{(\arabic{footnote})}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: nil
%%% End: 

